Fuel Saving Effect and Performance of Velocity Control for Modern Combustion-Powered Scooters

This paper investigates the performance and fuel-saving effect of a velocity control algorithm on modern 50 cc scooters (Euro 5). The European Parliament has adopted major CO$_2$ emission reductions by 2030. But modern combustion- powered scooters are inefficiently restricted and emit unnecessary amounts of CO$_2$. Replacing the original restriction method with the system presented in this paper, the engine's operating point is being improved significantly. Therefore, a Throttle-by-Wire-System senses the rider's throttle command and manipulates the throttle valve. A redundant wheel speed sensor measures the precise vehicle velocity using the magneto-resistive principle. The entire system is managed by a central ECU, executing the actual velocity control, fail-safe functions, power supply and handling inputs/outputs. For velocity control, an adaptive PI-controller has been simulated, virtually tuned and implemented, limiting the max. velocity regulated by legal constraints (45 km/h). In this way, the environmentally harmful restrictors used today can be bypassed. By implementing a human-machine interface, including a virtual dashboard, the system is capable of interfacing with the rider. For evaluation purposes a measurement box has been developed, logging vehicle orientation, system/control variables and engine parameters. A Peugeot Kisbee 50 4T (Euro 5) is serving as test vehicle. Finally, the system has been evaluated regarding performance and fuel efficiency both through simulation and road testing. Fuel savings of 13.6 % in real-world test scenarios were achieved while maintaining vehicle performance.

==> 1_intro.tex <==
\section{Introduction}
\IEEEPARstart{A}{ccording} to the climate targets of the European Climate Change Act, at least 55 \% of greenhouse gases are to be saved by 2030 compared to 1990 levels \cite{EUcca}. Considering the average distance traveled per inhabitant in the EU, the values vary between 5 and 20km a day. Depending on the country of origin, 57 \% to 81 \% of this daily distance is covered by car. Most often, the distance traveled by two-wheelers corresponds to less than 1\% \cite{EUpms}. However, for urban mobility, scooters are an excellent alternative. The potential for saving fuel and thus minimizing CO$_2$ emissions is enormous and can make a significant contribution to EU climate targets. Environmentally harmful 2-stroke engines are banned and the Euro 5 standard also applies to 50 cc scooters \cite{EURO5}. Comparing modern 4-stroke combustion and electrically powered scooters of Peugeot, Piaggio and Vespa, an average price for electric models of almost 160\% can be noticed. The difference in average range is even more striking, as the combustion engine exceeds that of the electric drive by a factor of 6. Especially when used in cities, users require longer ranges because frequent recharging is often difficult.\\

To fulfill Euro 5 requirements, modern combustion-powered scooters are equipped with gasoline injection and a catalytic converter \cite{Peugeot, Kymco}. To ensure optimal operation of the catalyst, the air/fuel mixture ($\lambda$) must be approx. 1 \cite{lambda}. Legal requirements state that 50 cc scooters cannot exceed a maximum speed of 45 km/h. By delaying the ignition timing, the engine is restricted in power, since reducing the fuel injected would cause $\lambda$ to become larger 1 (lean mixture). This can be solved by deactivating the original restriction of the test vehicle and applying a \ac{VC} algorithm. The basis is provided by a \ac{TbWS} \cite{TbWS_JK}, which enables electrical control of the throttle valve. For this purpose, the throttle position is sensed and the throttle valve is manipulated by an actuator. As a consequence, instead of the ignition timing, the airflow is regulated by means of the throttle valve position, which also results in a reduction of the fuel injection volume. This system can contribute substantially to reaching EU climate targets. To the best of our knowledge, this is the first approach of a \ac{VC} application on a modern 4-stroke 50 cc (Euro 5) scooter as an alternative restriction. The \ac{VC} system investigated here is intended to optimize fuel economy and improve exhaust emissions. \\

%The following novelties will make a significant scientific contribution in this class of vehicles:

\begin{itemize}
    \item By suppressing ignition timing manipulation, the engine efficiency is increased and the throttle valve opening can be reduced by almost 50 \% on level ground. 
    \item The controlled air supply minimizes the amount of fuel injected in line with the optimum stoichiometric ratio by up to approx. 20 \% on level ground.
    \item Based on the frequently maxed-out vehicle velocity, this alternative restriction significantly lowers fuel consumption/CO$_2$ emissions by 14 \%.
    \item Despite the minimized injection quantity, consistent vehicle performance can be demonstrated because the amount of energy supplied is used more effectively.
\end{itemize}


\subsection{Background on restricting methods}
Scooters are defined by EU law. In addition to the maximum speed of 45 km/h and the maximum engine capacity of 50 cc, the total power is also limited to 4 kW, regardless of the type of drive \cite{Def_scooter}. In most cases, vehicle performance is sufficient to reach higher speeds, so the surplus power above 45 km/h must be compensated. Generally, the surplus is still needed for heavy loads or inclines. In the past, mechanical restrictors were often used, which manipulated the flow behavior either through throttle orifices in the air intake or exhaust \cite{R1}. Limitation of the \ac{CVT} was particularly common, resulting in an unnecessarily high engine speed. Electronic throttling was opened with the arrival of electronic ignition. When the top speed was reached, the ignition was interrupted, resulting in the emission of unburned fuel. Modern powertrains have further capabilities to influence engine control due to gasoline injection. Injection volume and ignition timing are decisive here. Reducing the fuel supplied would be obvious, but leads to high combustion temperatures and interferes with the function of the catalytic converter \cite{R2}. As a consequence, engine damage and unacceptable exhaust emissions would be expected. Typically, ignition occurs 6° to 40° before the \ac{TDC}, depending on the engine speed. For restricting the top speed, the ignition timing is delayed towards the \ac{TDC} or even behind as shown in  Figure \ref{IgnT} (efficient left, restricted right). To achieve optimum efficiency, the maximum pressure must be reached shortly after \ac{TDC}. This ensures that the max. combustion chamber pressure can act on the piston from the start of expansion. By retarding the ignition timing, expansion is already taking place during combustion, thus reducing both the peak pressure and the usable expansion distance. The efficiency drops \cite{IgnT}.

\begin{figure}[!h]
\centering
\includegraphics[width=8.5cm]{Images/1_Intro_IgnT.pdf}
\caption{Ignition timing}
\label{IgnT}
\end{figure}

\subsection{Background on \acp{TbWS} \& velocity control }
\acp{TbWS} have been researched and integrated industrially to motorcycles \cite{TbWS_SportMotorbike, TbWS_BMW1, TbWS_BMW2}. A \ac{TbWS} has also been applied successfully to small-volume engines, coming with the minimum number of low-cost components, combined in the throttle body. The system is based on a throttle servo, throttle position sensor, throttle demand and speed sensor. To limit and adapt the engine speed in various load situations, the speed can be adjusted by an integral electronic control and resonant frequencies can be avoided. Besides the performance limitation, the system is capable of managing speed and load reductions during overheating. For cold starts, the idle speed can be adjusted on the outside temperature \cite{EngineManagement}. Also, an electronic throttle control for a 50cc two-stroke scooter application has been developed, improving fuel economy, idle-stability and implementing an electronic vehicle velocity control. By use of an electronic throttle control, the conventional \ac{CVT} restriction can be replaced, which leads to fuel savings of 22\% caused by the lowered engine speed. Additionally, the system allows controlling the idle engine speed after the start-up. The system is based on a carburetor-driven two-stroke scooter with a power of 4.2 kW and a twin variator pulley \ac{CVT} \cite{ETC_Peugeot}. Due to the mentioned powertrain, the system is not compliant with the Euro 5 standard. Nowadays systems use an originally optimal-designed \ac{CVT}. In addition, modern air-cooled four-strokes have a power output of max. 2.5kW due to the significantly lower power density. The potential within power surplus and transmission thus no longer exists. In addition, the fuel consumption of modern non-optimized scooter drives is considerably lower than that of an optimized 2-stroke \cite{2vs4-Stroke}. 
